OAT: Attesting Operation Integrity of Embedded Devices

Due to the wide adoption of IoT/CPS systems, embedded devices(IoT frontends) become increasingly connected and mission-critical, which in turn has attracted advanced attacks (e.g., control-flow hijacks and data-only attacks). Unfortunately, IoT backends are unable to detect if such attacks have happened while receiving data, service requests, or operation status from IoT devices. As a result, currently, IoT backends are forced to blindly trust the IoT devices that they interact with. To fill this void, we first formulate a new security property for embedded devices, called "Operation Execution Integrity" or OEI. We then design and build a system, OAT, that enables remote OEI attestation for ARM-based bare-metal embedded devices. Our formulation of OEI captures the integrity of both control flow and critical data involved in an operation execution. Therefore, satisfying OEI entails that an operation execution is free of unexpected control and data manipulations, which existing attestation methods cannot check. Our design of OAT strikes a balance between prover's constraints (embedded devices' limited computing power and storage) and verifier's requirements(complete verifiability and forensic assistance). OAT uses a new control-flow measurement scheme, which enables light-weight and space-efficient collection of measurements (97% space reduction from the trace-based approach). OAT performs the remote control-flow verification through abstract execution, which is fast and deterministic. OAT also features lightweight integrity checking for critical data (74% fewer instrumentation needed than previous work). Our security analysis shows that OAT allows remote verifiers or IoT backends to detect both control-flow hijacks and data-only attacks that affect the execution of operations on IoT devices. In our evaluation using real embedded programs, OAT incurs a runtime overhead of 2.7%.

==> Makefile <==
# Set this to one or more main LaTeX files (e.g. those with \documentclass) 
# for a specific build. Leave blank to build all files having an uncommented
# \documentclass.
MAIN=	


###########################################################################
#                 MAKE NO EDITS BELOW (except to debug)                   #
###########################################################################
#
#
# This is the PDFLATEX makefile, no support for ps/eps/dvi.
#
# Originally based on 
#   http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/Makefile
# but redeveloped by JG. Reuse by changing just the first line to list
# the main LaTeX source file.
#
# Features:
# - Finds all included LaTeX files, including includes within includes.
# - Finds all bibs and PDF figures included.
# - Automatically generates dependency information.
# - Repeats calls to PDFLATEX as necessary to fix cross references.
# - Displays missing references in a clean format at the end of the build.
# - Finds main LaTeX source files, so this makefile is reusable wihtout edits.
# - Works for files with bibliographies, and files without.

ifndef MAIN
MAIN:=	$(shell egrep -l "documentclass" *.tex)	
endif

ALLTEX:=$(shell ls *.tex)
ALLPDF:=$(ALLTEX:.tex=.pdf)

all pdf: $(MAIN:.tex=.pdf)
help ps dvi $(MAIN:.tex=.ps) $(MAIN:.tex=.dvi): die_unsupported
$(filter-out $(MAIN:.tex=.pdf),$(ALLPDF)): die_unsupported

%.pdf: %.fig
	rm -f $@
	fig2dev -L pdf $< > $@

%.aux: %.tex
	$(LATEX) $<

%.bbl: %.tex
	bibtex $(<:.tex=)
	$(LATEX) $<

%.pdf: %.aux
	@while (grep -q "Rerun to get" $(<:.aux=.log)) do \
		$(LATEX) $(<:.aux=.tex); \
	done
	@egrep -i "(Reference|Citation).*undefined" $(<:.aux=.log) ; true
	$(LATEX) $(<:.aux=.tex)

%.dep: %.tex
	@$(gettexs); $(getbibs); $(getfigs); \
	echo "$(<:.tex=.dep): Makefile " $$texs $$bibs $$figs > $@; \
	echo "$(<:.tex=.aux): " $$texs $$figs >> $@; \
	if [ $${#bibs} -gt 0 ]; then \
		echo "$(<:.tex=.bbl): " $$texs $$bibs >> $@; \
		echo "$(<:.tex=.pdf): $(<:.tex=.bbl)" >> $@; \
	fi

vpath %.fig figs

-include $(MAIN:.tex=.dep)

.PHONY: clean die_unsupported

double:
	for i in $(ALLTEX); do echo "Double words in $$i:" && ./double.pl < $$i; done

clean:
	rm -f *~ *.log *.aux *.dvi *.bbl *.blg *.cb *.dep $(TARGET)

copy:
	cp paper.pdf $(DESKTOP)/sp20-camera.pdf

die_unsupported:
	$(warning Unsupported Makefile build target. Supported targets are:)
	$(warning  <BLANK> all pdf $(TARGET) clean)
	$(error Exiting)

LATEX=	pdflatex #--interaction batchmode
#LATEX= latex2rtf #--interaction batchmode
TARGET=	$(MAIN:.tex=.pdf)

# 9 Dec 2008 JG: This is now a worklist algorithm to pick up all recursive
#   child dependencies of discovered includes.
define gettexs
  worklist="$< "; \
  while [ $${#worklist} -gt 0 ]; do \
    curr=$${worklist%% *}; \
    worklist=$${worklist#* }; \
    texs="$${texs}$$curr "; \
    worklist=$${worklist}`perl -ne '\
               ($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/; \
	       @_=split /,/; \
	       foreach $$t (@_) { \
	         if ($$t !~ /\.tex$$/) { $$t .= ".tex"; } \
                 if (-e $$t) { print "$$t " } \
	       }' $${curr}`; \
	done
endef

define getbibs
  bibs=`perl -ne '\
        ($$_)=/^[^%]*\\\bibliography\{(.*?)\}/; \
        @_=split /,/; \
        foreach $$b (@_) { \
          if (-e "$$b.bib") { print "$$b.bib " } \
        }' $$texs`
endef

define getfigs
  figs=`perl -ne '\
        ($$_)=/^[^%]*\\\includegraphics(?:\[.*?\])?\{(.*?)\}/g; \
        if (defined($$_)) { \
          if ($$_ !~ /\.pdf$$/) { $$_ .= ".pdf"; } \
          if (-e $$_) { print "$$_ "; } \
        }' $$texs`
endef


==> sec.tex <==
\section{Security Considerations}
\label{sec:security}
Our threat model (\S~\ref{sec:threatModel}) anticipates that attackers may find
and exploit unknown vulnerabilities in the code running in the Normal World.
However, dynamic code injection or modification is disallowed, which the
existing code integrity schemes for embedded devices can
enforce~\cite{clements2017protecting,kimsecuring}.  



To evade \toolname, a normal-world attacker would need to \textcircled{1}
disable the instrumentation or the trampolines, or \textcircled{2} abuse the
interfaces that the measurement engine exposed to the trampolines, or CA-TA
interfaces, or \textcircled{3} manipulate the control flow to find a HASH
collision, thus bypassing the verification, or \textcircled{4} modify the attestation
blob including replay an old recorded blob.  
Without the ability to inject new code or modify the instrumented code
(explained earlier), the attacker cannot directly escape or remove the inline
instrumentation or the trampolines. Moreover, any attempt to force an executing
operation to skip an instrumentation site (via  control-flow manipulation) is
caught by the OEI attestation. Therefore, \textcircled{1} is prevented. 

To stop \textcircled{2}, our design ensures that only the trampoline functions
can directly invoke the CA-TA interfaces and the rest of the code in the Normal
World cannot. This is achieved as follows. The compiler disallows
world-switching instructions ({\tt smc}) outside of the trampoline library
(i.e., only the library can directly initiate the switch and invoke the CA-TA
interface). To further prevent code reuse attacks (e.g., jumping to the
interface invocation point in the library from outside), \toolname loads the
library in a designated memory region; the compiler masks the target of every
indirect control transfer in the embedded program so that the trampoline library
cannot be reached via indirect calls or jumps or returns (i.e., only hard-coded
direct calls from each instrumentation site can reach trampolines).
This masking-based technique is highly efficient and is
commonly used for software fault isolation. As a result, \textcircled{2}
is prevented. 

With a collision analysis, we will see \textcircled{3} is not possible
even with offline brute force attack. 
Assuming the attacker may exploit memory error and overwrite return address on stack 
in arbitrary way to 
change the control flow to attacker's favor. As a result, every change will be reflected
in the return event history, of which our HASH is calculated upon. To bypass the
check, the attacker needs to find a different return history that hit a collision of 
a given return history. It's equivalent to
find another input B to the BLAKE-2 HASH function that has the same HASH value for a given
input A. Considering the HASH output is 32 Bytes, the attacker has $40\%$ chance of collisions
when hashing  $2^{128}$ or $10^{30}$ billion items, assuming the output of BLAKE-2 is evenly 
distributed. 


For \textcircled{4}, as the integrity of the attestation is guarded by a signature that generated
from TEE with the provisioned private key, it's easy for the verifier to check
the signature. Replay attack is prevented by including a fresh nounce 
generated by the attestation requester into our attestation blob. 


There is no higher privileged code (e.g., a standalone OS) that needs to be
protected or trusted because \toolname targets bare-metal embedded devices. 
For the same reason, it is realistic to require the monolithic binary to be
entirely built using \toolname compiler. 


==> security_analysis.tex <==
1) messing up our CA/TA interfaces.
Our OAT system consists of instrumented application running in the
normal world and the trusted application(TA) running in the secure
world. User application will do a world switch through our trampoline
function to secure world and take measurements for the data and control
event. As we assume Data Execution Prevention(DEP) is there, so the
attacker can't overwrite our trampoline function call to remove the
attestation code, but it can try to launch ROP attack and call smc
instruction directly so that they can mess up our measurements by feeding
fake parameters to smc calls.

In order to prevent ROP attack on launching direct smc calls, we need
to prevent control hijacking through indirect call or function return
that jump directly to our smc calls. Since we are in control of the
instrumentation of indirect calls and function returns, we can mask 
the target address to confine it to a known range that only 
contain the application code, the smc call is out of reach for the
indirect control transfers. As for our trampolines, we call the entrance
of smc calls through direct function calls.

If the attacker is in control of the stack, she may want to launch an
ROP attack to our instrumentation site through stack smashing,
however, return instructions are instrumented, and they will be encoded
into the HASH value for verification, so it will finally be caught at
verification time. If the attacker try to manipulate function pointer,
it will also be recorded in our control flow stream, and will finally
be verified against CFG at Verifier side.

2) DOP attack.
The attacker may turn to control flow bending by launching DOP attack,
which don't violate the CFG. However, DOP attack relies on dispatcher
function which usually can change its own return address, but it
will be caught by our return address HASH, that's because when we
reconstruct the execution at Verifier side, we will detect such attack
that a function return to the start address of itself. DOP attack is
also possible on pure program data, however, due to our critical data
integrity check, the attack on data can only be successful on non-critical
program data whose affect to the application is restrained to limited
level.

On the other hand, DOP attack features manipulating control dependent
data, which can bend the control flow without violating CFG, however,
our compiler automatically annotate the control dependent data as 
critical data, so that our CVI check will prevent this kind of manipulation. 

Our defense on DOP attack shows that we have a stricter check by
reconstruct the execution of program at prover side and can detect
more attack than normal CFI protection. And we introduce limited
space overhead by using HASH based on verification on return address.

